Understanding Semantic IDs: From Item Representation to Item Selection in Generative Recommendation

Semantic IDs (SIDs) are now a central component of generative recommendation. Current SID-based systems assign three roles to the same token sequence. Shared prefixes are intended to organize related items, the complete SID identifies an individual item, and each generated token narrows the items that can still be returned. We systematically investigate SIDs from item encoding and SID construction to autoregressive generation and final recommendation. We examine how SID construction changes item representations and how those changes affect generation. Across three Amazon domains and eight SID constructions, SID neighborhoods recover only 32.2% of the encoder's ten nearest neighbors on average. Alternative item descriptions still retrieve the corresponding item first in 99.57% of controlled cases, yet change 38.4% of exact SIDs. These results show that SIDs retain broad organization but lose much of the encoder's fine local structure, while their exact tokens are not determined by item meaning alone. This loss becomes consequential during generation. After the final semantic token, TIGER retains only 29.9% of held-out targets that were plausible recommendations before SID filtering. Motivated by these findings, we propose Item-Supported Decoding (ISD), a lightweight inference-time method that allows a user-specific item ranking to support corresponding SID prefixes before beam search discards them. The same ranking then orders the generated items. ISD requires no additional parameters or retraining of the SID constructor or decoder. We empirically show that ISD improves NDCG@10 over the corresponding SID backbone in every evaluated setting, with relative gains of up to 31.2%. Our results show that SIDs provide useful coarse item organization, but their fine boundaries should not alone determine which items remain available during generation.

==> contents/A_table_definitions.tex <==
% Table macros used only by the appendix.
\newcommand{\capacitytable}{%
\begin{table*}[t]
  \centering
  \caption{Capacity coverage (percent): exact code changed / original encoder
  top-10 neighbors recovered by the code. Larger three-level codebooks
  generally preserve more of the encoder's fine neighborhood but also make
  exact tokens more dependent on description form. \textbf{TBD} cells are
  runnable. Completing the Baby and Yelp rows would complete the common-grid
  sweep; Electronics is an optional scale extension.}
  \label{tab:capacity}
  \small
  \setlength{\tabcolsep}{5.0pt}
  \begin{tabular}{llrrr}
    \toprule
    Dataset & Constructor & $3\times16$ & $3\times64$ & $3\times256$ \\
    \midrule
    Baby & L2 RQ-KMeans & TBD & TBD & 17.4 / 38.9 \\
    Baby & RQ-VAE & TBD & TBD & 54.5 / 19.9 \\
    Office & L2 RQ-KMeans & 15.6 / 7.8 & 21.2 / 20.6 & 24.6 / 33.1 \\
    Office & RQ-VAE & 31.5 / 2.4 & 43.8 / 7.4 & 53.9 / 13.8 \\
    Scientific & L2 RQ-KMeans & 11.1 / 18.3 & 14.3 / 33.3 & 14.0 / 45.1 \\
    Scientific & RQ-VAE & 29.7 / 8.7 & 37.2 / 15.7 & 45.7 / 32.8 \\
    Yelp & L2 RQ-KMeans & TBD & TBD & TBD \\
    Yelp & RQ-VAE & TBD & TBD & TBD \\
    Electronics & L2 RQ-KMeans & TBD & TBD & 15.7 / 15.0 \\
    Electronics & RQ-VAE & TBD & TBD & 50.3 / 9.8 \\
    \bottomrule
  \end{tabular}
\end{table*}
}

\newcommand{\nativeneighborhoodtable}{%
\begin{table*}[t]
  \centering
  \caption{Native-system representation coverage against the agreed dataset
  grid. A completed numeric cell reports \emph{exact code changed / encoder
  neighbors recovered by the code / code neighbors retained between
  descriptions}, in percent. Baby, Office, Scientific, and Yelp are the
  common target datasets; Electronics is a separate scale check. Results on
  release-specific datasets are isolated in ``native-only.'' \textbf{TBD}
  denotes a runnable faithful cell; \textbf{X} denotes a cell blocked by
  unavailable released artifacts.}
  \label{tab:native-neighborhood}
  \scriptsize
  \setlength{\tabcolsep}{2.6pt}
  \begin{tabular}{lcccccp{0.20\textwidth}p{0.21\textwidth}}
    \toprule
    Native construction & Baby & Office & Scientific & Yelp & Electronics
      & Native-only completed cell & Status explanation \\
    \midrule
    Offline residual SID (BERT)
      & TBD & 18.1/36.3/91.9 & 11.8/44.3/97.8 & TBD & TBD &
      & Baby, Yelp, and Electronics native cells not run \\
    RPG parallel SID
      & X & X & X & X & X & Beauty: 86.8/55.4/87.3
      & Required native embeddings/provenance unavailable on common datasets \\
    DIGER joint SID
      & X & X & X & X & X & Instruments: 82.7/30.3/60.1
      & I-Shop is paper-fidelity validated; B-Shop and Yelp reproduce the
        official-code seed-0 pipeline; the editable constructor remains unavailable \\
    SIDReasoner
      & X & X & X & X & X &
      & Exact description template, encoder, codebooks, and suffix policy unavailable \\
    MiniOneRec
      & X & X & X & X & X &
      & Unreleased trained codebook \\
    \bottomrule
  \end{tabular}
\end{table*}
}

\newcommand{\decoderbreadthtable}{%
\begin{table*}[t]
  \centering
  \caption{Decoder coverage on the same agreed dataset grid. Completed cells
  state the decoder-side evidence. \textbf{TBD} denotes a runnable training or
  evaluation cell; \textbf{X} is blocked by a missing constructor or prediction
  checkpoint. Release-specific datasets are isolated in ``native-only.''
  SIDReasoner is a next-token diagnostic, not an alternate-code test.}
  \label{tab:decoder-breadth}
  \scriptsize
  \setlength{\tabcolsep}{2.6pt}
  \begin{tabular}{lcccccp{0.20\textwidth}p{0.22\textwidth}}
    \toprule
    Decoder & Baby & Office & Scientific & Yelp & Electronics
      & Native-only completed cell & Unfinished or blocked \\
    \midrule
    Offline residual SID
      & Lockout $\approx100\%$ & Lockout 100\% & Lockout 100\% & TBD & TBD &
      & Alternate-route H@50 is 0--.0003; aliases restore the learned route \\
    DIGER
      & TBD & TBD & TBD & Baseline done & TBD
      & Instruments: lockout 98.59\%, NDCG $-15.4\%$; I-Shop fidelity validated
      & B-Shop/Yelp analyses TBD; editable constructor and popularity slices unavailable \\
    SIDReasoner~\cite{sidreasoner2026}
      & X & Prefix diagnostic & X & X & X & Games/Industrial: prefix diagnostic
      & Exact constructor unavailable; no alternate-code test \\
    MiniOneRec
      & X & X & X & X & X & Office/Scientific: checkpoint fidelity only
      & Unreleased trained codebook blocks target-side test \\
    RPG
      & X & X & X & X & X &
      & No prediction checkpoint released \\
    \bottomrule
  \end{tabular}
\end{table*}
}

\newcommand{\continuousreferencetable}{%
\begin{table*}[t]
  \centering
  \caption{Continuous-recommender reference. Base metric ranges are across
  three seeds; brackets for changes and retention are 95\% intervals.
  \textbf{TBD} rows are runnable. Baby and Yelp are the missing common-grid
  references; Electronics is an optional scale extension.}
  \label{tab:continuous-reference}
  \small
  \setlength{\tabcolsep}{4.0pt}
  \begin{tabular}{lrrrrr}
    \toprule
    Dataset & Base H@10 & Base N@10 & $\Delta$H@10 & $\Delta$N@10
      & Original-hit retention \\
    \midrule
    Baby & \multicolumn{5}{c}{TBD} \\
    Office & .0909--.0919 & .0637--.0643
      & -.00720 [-.00808, -.00633] & -.01047 [-.01090, -.00999]
      & .8685 [.8633, .8737] \\
    Scientific & .0788--.0801 & .0466--.0497
      & -.00544 [-.00807, -.00246] & -.00290 [-.00436, -.00126]
      & .8486 [.8300, .8672] \\
    Yelp & \multicolumn{5}{c}{TBD} \\
    Electronics & \multicolumn{5}{c}{TBD (optional scale check)} \\
    \bottomrule
  \end{tabular}
\end{table*}
}

